The layered phase of anisotropic gauge theories: A model for topological insulators

Topological insulators are materials where current does not flow through the bulk, but along the boundaries, only. They are of particular practical importance, since it is considerably more difficult, by ``conventional'' means, to affect their transport properties, than for the case of conventional materials. They are, thus, particularly robust to perturbations. One way to accomplish such changes is by engineering defects. The defects that have been the most studied are domain walls; however flux compactifications can, also, work. We recall the domain wall construction and compare it to the construction from flux compactification. A particular way of engineering the presence of such defects is by introducing anisotropic couplings for the gauge fields. In this case a new phase appears, where matter is confined along layers and local degrees of freedom cannot propagate through the bulk. It is, also, possible to take into account the ``backreaction'' of the dynamics of the gauge fields on the defects and find that a new phase, the layered phase, where, while transport of local degrees of freedom is confined to surfaces, the topological properties can propagate through the bulk, constituting an example of anomaly flow. The anisotropy itself can be understood as emerging from a particular Maxwell--dilaton coupling.

==> fermions3.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.175pt]{0.350pt}{0.350pt}}%
\begin{picture}(1500,900)(0,0)
%\tenrm
\sbox{\plotpoint}{\rule[-0.175pt]{0.350pt}{0.350pt}}%
\put(264,158){\rule[-0.175pt]{282.335pt}{0.350pt}}
\put(264,158){\rule[-0.175pt]{0.350pt}{151.526pt}}
\put(264,158){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,158){\makebox(0,0)[r]{0}}
\put(1416,158){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,221){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,221){\makebox(0,0)[r]{0.2}}
\put(1416,221){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,284){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,284){\makebox(0,0)[r]{0.4}}
\put(1416,284){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,347){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,347){\makebox(0,0)[r]{0.6}}
\put(1416,347){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,410){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,410){\makebox(0,0)[r]{0.8}}
\put(1416,410){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,473){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,473){\makebox(0,0)[r]{1}}
\put(1416,473){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,535){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,535){\makebox(0,0)[r]{1.2}}
\put(1416,535){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,598){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,598){\makebox(0,0)[r]{1.4}}
\put(1416,598){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,661){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,661){\makebox(0,0)[r]{1.6}}
\put(1416,661){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,724){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,724){\makebox(0,0)[r]{1.8}}
\put(1416,724){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,787){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(242,787){\makebox(0,0)[r]{2}}
\put(1416,787){\rule[-0.175pt]{4.818pt}{0.350pt}}
\put(264,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(264,113){\makebox(0,0){0}}
\put(264,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(394,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(394,113){\makebox(0,0){0.2}}
\put(394,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(524,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(524,113){\makebox(0,0){0.4}}
\put(524,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(655,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(655,113){\makebox(0,0){0.6}}
\put(655,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(785,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(785,113){\makebox(0,0){0.8}}
\put(785,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(915,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(915,113){\makebox(0,0){1}}
\put(915,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1045,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1045,113){\makebox(0,0){1.2}}
\put(1045,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1176,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1176,113){\makebox(0,0){1.4}}
\put(1176,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1306,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1306,113){\makebox(0,0){1.6}}
\put(1306,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1436,158){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(1436,113){\makebox(0,0){1.8}}
\put(1436,767){\rule[-0.175pt]{0.350pt}{4.818pt}}
\put(264,158){\rule[-0.175pt]{282.335pt}{0.350pt}}
\put(1436,158){\rule[-0.175pt]{0.350pt}{151.526pt}}
\put(264,787){\rule[-0.175pt]{282.335pt}{0.350pt}}
\put(45,472){\makebox(0,0)[l]{\shortstack{$\beta$}}}
\put(850,68){\makebox(0,0){$\beta'$}}
\put(394,476){\makebox(0,0)[l]{$\diamond$}}
\put(459,284){\makebox(0,0)[l]{Strong}}
\put(915,473){\makebox(0,0)[l]{Weak}}
\put(329,598){\makebox(0,0)[l]{Layered}}
\put(264,158){\rule[-0.175pt]{0.350pt}{151.526pt}}
\put(433,693){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(433,630){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(440,535){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(446,504){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(459,441){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(472,410){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(590,378){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(707,378){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(817,347){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(889,315){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(1006,284){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\put(1091,252){\raisebox{-1.2pt}{\makebox(0,0){$\Diamond$}}}
\sbox{\plotpoint}{\rule[-0.350pt]{0.700pt}{0.700pt}}%
\put(440,787){\usebox{\plotpoint}}
\put(440,650){\rule[-0.350pt]{0.700pt}{32.883pt}}
\put(441,640){\rule[-0.350pt]{0.700pt}{2.529pt}}
\put(442,629){\rule[-0.350pt]{0.700pt}{2.529pt}}
\put(443,619){\rule[-0.350pt]{0.700pt}{2.529pt}}
\put(444,608){\rule[-0.350pt]{0.700pt}{2.529pt}}
\put(445,598){\rule[-0.350pt]{0.700pt}{2.529pt}}
\put(446,530){\rule[-0.350pt]{0.700pt}{16.326pt}}
\put(447,525){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(448,520){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(449,515){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(450,511){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(451,506){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(452,501){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(453,496){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(454,492){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(455,487){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(456,482){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(457,477){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(458,473){\rule[-0.350pt]{0.700pt}{1.149pt}}
\put(459,470){\usebox{\plotpoint}}
\put(460,468){\usebox{\plotpoint}}
\put(461,465){\usebox{\plotpoint}}
\put(462,463){\usebox{\plotpoint}}
\put(463,460){\usebox{\plotpoint}}
\put(464,458){\usebox{\plotpoint}}
\put(465,456){\usebox{\plotpoint}}
\put(466,453){\usebox{\plotpoint}}
\put(467,451){\usebox{\plotpoint}}
\put(468,448){\usebox{\plotpoint}}
\put(469,446){\usebox{\plotpoint}}
\put(470,443){\usebox{\plotpoint}}
\put(471,441){\usebox{\plotpoint}}
\put(472,439){\usebox{\plotpoint}}
\put(473,436){\usebox{\plotpoint}}
\put(474,434){\usebox{\plotpoint}}
\put(475,431){\usebox{\plotpoint}}
\put(476,429){\usebox{\plotpoint}}
\put(477,426){\usebox{\plotpoint}}
\put(478,424){\usebox{\plotpoint}}
\put(479,422){\usebox{\plotpoint}}
\put(480,419){\usebox{\plotpoint}}
\put(481,417){\usebox{\plotpoint}}
\put(482,414){\usebox{\plotpoint}}
\put(483,412){\usebox{\plotpoint}}
\put(484,410){\usebox{\plotpoint}}
\put(485,410){\usebox{\plotpoint}}
\put(485,410){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(490,409){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(495,408){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(501,407){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(506,406){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(512,405){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(517,404){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(523,403){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(528,402){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(534,401){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(539,400){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(545,399){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(550,398){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(556,397){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(561,396){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(567,395){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(572,394){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(578,393){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(583,392){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(589,391){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(594,390){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(600,389){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(605,388){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(610,387){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(616,386){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(621,385){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(627,384){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(632,383){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(638,382){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(643,381){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(649,380){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(654,379){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(660,378){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(665,377){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(671,376){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(676,375){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(682,374){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(687,373){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(693,372){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(698,371){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(704,370){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(709,369){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(715,368){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(720,367){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(725,366){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(731,365){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(736,364){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(742,363){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(747,362){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(753,361){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(758,360){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(764,359){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(769,358){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(775,357){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(780,356){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(786,355){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(791,354){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(797,353){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(802,352){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(808,351){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(813,350){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(819,349){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(824,348){\rule[-0.350pt]{1.319pt}{0.700pt}}
\put(830,347){\usebox{\plotpoint}}
\put(832,346){\usebox{\plotpoint}}
\put(835,345){\usebox{\plotpoint}}
\put(838,344){\usebox{\plotpoint}}
\put(841,343){\usebox{\plotpoint}}
\put(844,342){\usebox{\plotpoint}}
\put(847,341){\usebox{\plotpoint}}
\put(850,340){\usebox{\plotpoint}}
\put(853,339){\usebox{\plotpoint}}
\put(856,338){\usebox{\plotpoint}}
\put(859,337){\usebox{\plotpoint}}
\put(861,336){\usebox{\plotpoint}}
\put(864,335){\usebox{\plotpoint}}
\put(867,334){\usebox{\plotpoint}}
\put(870,333){\usebox{\plotpoint}}
\put(873,332){\usebox{\plotpoint}}
\put(876,331){\usebox{\plotpoint}}
\put(879,330){\usebox{\plotpoint}}
\put(882,329){\usebox{\plotpoint}}
\put(885,328){\usebox{\plotpoint}}
\put(888,327){\usebox{\plotpoint}}
\put(891,326){\usebox{\plotpoint}}
\put(893,325){\usebox{\plotpoint}}
\put(896,324){\usebox{\plotpoint}}
\put(899,323){\usebox{\plotpoint}}
\put(902,322){\usebox{\plotpoint}}
\put(905,321){\usebox{\plotpoint}}
\put(908,320){\usebox{\plotpoint}}
\put(911,319){\usebox{\plotpoint}}
\put(914,318){\usebox{\plotpoint}}
\put(917,317){\usebox{\plotpoint}}
\put(920,316){\usebox{\plotpoint}}
\put(922,315){\usebox{\plotpoint}}
\put(925,314){\usebox{\plotpoint}}
\put(928,313){\usebox{\plotpoint}}
\put(931,312){\usebox{\plotpoint}}
\put(934,311){\usebox{\plotpoint}}
\put(937,310){\usebox{\plotpoint}}
\put(940,309){\usebox{\plotpoint}}
\put(943,308){\usebox{\plotpoint}}
\put(946,307){\usebox{\plotpoint}}
\put(949,306){\usebox{\plotpoint}}
\put(952,305){\usebox{\plotpoint}}
\put(954,304){\usebox{\plotpoint}}
\put(957,303){\usebox{\plotpoint}}
\put(960,302){\usebox{\plotpoint}}
\put(963,301){\usebox{\plotpoint}}
\put(966,300){\usebox{\plotpoint}}
\put(969,299){\usebox{\plotpoint}}
\put(972,298){\usebox{\plotpoint}}
\put(975,297){\usebox{\plotpoint}}
\put(978,296){\usebox{\plotpoint}}
\put(981,295){\usebox{\plotpoint}}
\put(983,294){\usebox{\plotpoint}}
\put(986,293){\usebox{\plotpoint}}
\put(989,292){\usebox{\plotpoint}}
\put(992,291){\usebox{\plotpoint}}
\put(995,290){\usebox{\plotpoint}}
\put(998,289){\usebox{\plotpoint}}
\put(1001,288){\usebox{\plotpoint}}
\put(1004,287){\usebox{\plotpoint}}
\put(1007,286){\usebox{\plotpoint}}
\put(1010,285){\usebox{\plotpoint}}
\put(1013,284){\usebox{\plotpoint}}
\put(1015,283){\usebox{\plotpoint}}
\put(1018,282){\usebox{\plotpoint}}
\put(1021,281){\usebox{\plotpoint}}
\put(1024,280){\usebox{\plotpoint}}
\put(1026,279){\usebox{\plotpoint}}
\put(1029,278){\usebox{\plotpoint}}
\put(1032,277){\usebox{\plotpoint}}
\put(1035,276){\usebox{\plotpoint}}
\put(1038,275){\usebox{\plotpoint}}
\put(1040,274){\usebox{\plotpoint}}
\put(1043,273){\usebox{\plotpoint}}
\put(1046,272){\usebox{\plotpoint}}
\put(1049,271){\usebox{\plotpoint}}
\put(1052,270){\usebox{\plotpoint}}
\put(1054,269){\usebox{\plotpoint}}
\put(1057,268){\usebox{\plotpoint}}
\put(1060,267){\usebox{\plotpoint}}
\put(1063,266){\usebox{\plotpoint}}
\put(1066,265){\usebox{\plotpoint}}
\put(1068,264){\usebox{\plotpoint}}
\put(1071,263){\usebox{\plotpoint}}
\put(1074,262){\usebox{\plotpoint}}
\put(1077,261){\usebox{\plotpoint}}
\put(1080,260){\usebox{\plotpoint}}
\put(1082,259){\usebox{\plotpoint}}
\put(1085,258){\usebox{\plotpoint}}
\put(1088,257){\usebox{\plotpoint}}
\put(1091,256){\usebox{\plotpoint}}
\put(1094,255){\usebox{\plotpoint}}
\put(1096,254){\usebox{\plotpoint}}
\put(1099,253){\usebox{\plotpoint}}
\put(1102,252){\usebox{\plotpoint}}
\put(1105,251){\usebox{\plotpoint}}
\put(1107,250){\usebox{\plotpoint}}
\put(1110,249){\usebox{\plotpoint}}
\put(1113,248){\usebox{\plotpoint}}
\put(1116,247){\usebox{\plotpoint}}
\put(1119,246){\usebox{\plotpoint}}
\put(1121,245){\usebox{\plotpoint}}
\put(1124,244){\usebox{\plotpoint}}
\put(1127,243){\usebox{\plotpoint}}
\put(1130,242){\usebox{\plotpoint}}
\put(1133,241){\usebox{\plotpoint}}
\put(1135,240){\usebox{\plotpoint}}
\put(1138,239){\usebox{\plotpoint}}
\put(1141,238){\usebox{\plotpoint}}
\put(1144,237){\usebox{\plotpoint}}
\put(1147,236){\usebox{\plotpoint}}
\put(1149,235){\usebox{\plotpoint}}
\put(1152,234){\usebox{\plotpoint}}
\put(1155,233){\usebox{\plotpoint}}
\put(1158,232){\usebox{\plotpoint}}
\put(1161,231){\usebox{\plotpoint}}
\put(1163,230){\usebox{\plotpoint}}
\put(1166,229){\usebox{\plotpoint}}
\put(1169,228){\usebox{\plotpoint}}
\put(1172,227){\usebox{\plotpoint}}
\put(1175,226){\usebox{\plotpoint}}
\put(1177,225){\usebox{\plotpoint}}
\put(1180,224){\usebox{\plotpoint}}
\put(1183,223){\usebox{\plotpoint}}
\put(1186,222){\usebox{\plotpoint}}
\put(1189,221){\usebox{\plotpoint}}
\put(1191,220){\usebox{\plotpoint}}
\put(1193,219){\usebox{\plotpoint}}
\put(1195,218){\usebox{\plotpoint}}
\put(1197,217){\usebox{\plotpoint}}
\put(1199,216){\usebox{\plotpoint}}
\put(1201,215){\usebox{\plotpoint}}
\put(1204,214){\usebox{\plotpoint}}
\put(1206,213){\usebox{\plotpoint}}
\put(1208,212){\usebox{\plotpoint}}
\put(1210,211){\usebox{\plotpoint}}
\put(1212,210){\usebox{\plotpoint}}
\put(1214,209){\usebox{\plotpoint}}
\put(1217,208){\usebox{\plotpoint}}
\put(1219,207){\usebox{\plotpoint}}
\put(1221,206){\usebox{\plotpoint}}
\put(1223,205){\usebox{\plotpoint}}
\put(1225,204){\usebox{\plotpoint}}
\put(1227,203){\usebox{\plotpoint}}
\put(1230,202){\usebox{\plotpoint}}
\put(1232,201){\usebox{\plotpoint}}
\put(1234,200){\usebox{\plotpoint}}
\put(1236,199){\usebox{\plotpoint}}
\put(1238,198){\usebox{\plotpoint}}
\put(1240,197){\usebox{\plotpoint}}
\put(1242,196){\usebox{\plotpoint}}
\put(1245,195){\usebox{\plotpoint}}
\put(1247,194){\usebox{\plotpoint}}
\put(1249,193){\usebox{\plotpoint}}
\put(1251,192){\usebox{\plotpoint}}
\put(1253,191){\usebox{\plotpoint}}
\put(1255,190){\usebox{\plotpoint}}
\put(1258,189){\usebox{\plotpoint}}
\put(1260,188){\usebox{\plotpoint}}
\put(1262,187){\usebox{\plotpoint}}
\put(1264,186){\usebox{\plotpoint}}
\put(1266,185){\usebox{\plotpoint}}
\put(1268,184){\usebox{\plotpoint}}
\put(1271,183){\usebox{\plotpoint}}
\put(1273,182){\usebox{\plotpoint}}
\put(1275,181){\usebox{\plotpoint}}
\put(1277,180){\usebox{\plotpoint}}
\put(1279,179){\usebox{\plotpoint}}
\put(1281,178){\usebox{\plotpoint}}
\put(1283,177){\usebox{\plotpoint}}
\put(1286,176){\usebox{\plotpoint}}
\put(1288,175){\usebox{\plotpoint}}
\put(1290,174){\usebox{\plotpoint}}
\put(1292,173){\usebox{\plotpoint}}
\put(1294,172){\usebox{\plotpoint}}
\put(1296,171){\usebox{\plotpoint}}
\put(1299,170){\usebox{\plotpoint}}
\put(1301,169){\usebox{\plotpoint}}
\put(1303,168){\usebox{\plotpoint}}
\put(1305,167){\usebox{\plotpoint}}
\put(1307,166){\usebox{\plotpoint}}
\put(1309,165){\usebox{\plotpoint}}
\put(1312,164){\usebox{\plotpoint}}
\put(1314,163){\usebox{\plotpoint}}
\put(1316,162){\usebox{\plotpoint}}
\put(1318,161){\usebox{\plotpoint}}
\put(1320,160){\usebox{\plotpoint}}
\put(1322,159){\usebox{\plotpoint}}
\put(1324,158){\usebox{\plotpoint}}
\sbox{\plotpoint}{\rule[-0.500pt]{1.000pt}{1.000pt}}%
\put(329,410){\makebox(0,0){$+$}}
\put(394,410){\makebox(0,0){$+$}}
\put(459,410){\makebox(0,0){$+$}}
\put(524,410){\makebox(0,0){$+$}}
\sbox{\plotpoint}{\rule[-0.350pt]{0.700pt}{0.700pt}}%
\put(264,410){\usebox{\plotpoint}}
\put(264,410){\rule[-0.350pt]{3.915pt}{0.700pt}}
\put(280,409){\rule[-0.350pt]{3.915pt}{0.700pt}}
\put(296,408){\rule[-0.350pt]{3.915pt}{0.700pt}}
\put(312,407){\rule[-0.350pt]{3.915pt}{0.700pt}}
\put(329,406){\rule[-0.350pt]{36.536pt}{0.700pt}}
\put(480,405){\rule[-0.350pt]{5.219pt}{0.700pt}}
\put(502,404){\rule[-0.350pt]{5.220pt}{0.700pt}}
\end{picture}

